Learning Task Specifications from Demonstrations

Real world applications often naturally decompose into several sub-tasks. In many settings (e.g., robotics) demonstrations provide a natural way to specify the sub-tasks. However, most methods for learning from demonstrations either do not provide guarantees that the artifacts learned for the sub-tasks can be safely recombined or limit the types of composition available. Motivated by this deficit, we consider the problem of inferring Boolean non-Markovian rewards (also known as logical trace properties or specifications) from demonstrations provided by an agent operating in an uncertain, stochastic environment. Crucially, specifications admit well-defined composition rules that are typically easy to interpret. In this paper, we formulate the specification inference task as a maximum a posteriori (MAP) probability inference problem, apply the principle of maximum entropy to derive an analytic demonstration likelihood model and give an efficient approach to search for the most likely specification in a large candidate pool of specifications. In our experiments, we demonstrate how learning specifications can help avoid common problems that often arise due to ad-hoc reward composition.

==> intro.tex <==
\section{Introduction}
% Setup MDPS and IRL
In many settings (e.g., robotics) demonstrations provide a natural way
to specify a task. For example, an agent (e.g., human expert) gives
one or more demonstrations of the task from which we seek to
automatically synthesize a policy for the robot to execute.
Typically, one models the demonstrator as episodically operating
within a dynamical system whose transition relation only depends on
the current state and action (called the Markov
condition). However, even if the dynamics are Markovian, many
problems are naturally modeled in non-Markovian terms (see
Ex~\ref{ex:intro}).\vspace{4px}
\fbox{
\begin{minipage}[c]{0.97\textwidth}
  \noindent
  \begin{minipage}{0.7\textwidth}
    \begin{example}\label{ex:intro}
      Consider the task illustrated in Figure~\ref{fig:gridworld}. In
      this task, the agent moves in a discrete gridworld and can take
      actions to move in the cardinal directions (north, south, east,
      west). Further, the agent can sense abstract features of the
      domain represented as colors. The task is to reach any of the
      yellow (recharge) tiles without touching a red tile (lava) -- we
      refer to this sub-task as YR. Additionally, if a blue tile
      (water) is stepped on, the agent must step on a brown tile
      (drying tile) before going to a yellow tile -- we refer to this
      sub-task as BBY.  The last constraint requires recall of two
      state bits of history (and is thus not Markovian): one bit for whether
      the robot is wet and another bit encoding if the robot recharged
      while wet.
    \end{example}
  \end{minipage}
  \hfill
  \begin{minipage}[c]{0.25\textwidth}
    \begin{Figure}
      \centering
      \includegraphics[width=\linewidth]{imgs/simple_gridworld_doshow}
      \captionof{figure}{\label{fig:gridworld}}
    \end{Figure}
  \end{minipage}
\end{minipage}
}

Further, like Ex~\ref{ex:intro}, many tasks are naturally decomposed
into several sub-tasks. This work aims to address the question of how
to systematically and separately learn non-Markovian sub-tasks such
that they can be readily and safely recomposed into the larger
meta-task.

Here, we argue that \textit{non-Markovian Boolean specifications} provide
a powerful, flexible, and easily transferable formalism for task
representations when learning from demonstrations. This stands in
contrast to the quantitative scalar reward functions commonly 
associated with Markov Decision Processes. 
%In particular, focusing on
%Boolean specifications has two key benefits: (1) The ability to
%naturally express tasks with \textit{temporal dependencies} and (2)
%the ability to take advantage of the \textit{compositionality} that is
%present in many problems.
Focusing on Boolean specifications has certain benefits: 
(1) The ability to naturally express tasks with \textit{temporal dependencies};
(2) the ability to take advantage of the \textit{compositionality} 
present in many problems, and
(3) use of {\em formal methods} for planning and verification~\cite{seshia-arxiv16}.

Although standard quantitative scalar reward functions could be used
to learn this task from demonstrations, three issues arise.  First,
consider the problem of \textit{temporal specifications}: reward
functions are typically Markovian, so requirements like those in
Ex~\ref{ex:intro} cannot be directly expressed in the task
representation. One could explicitly encode time into a state and
reduce the problem to learning a Markovian reward on new
time-dependent dynamics; however, in general, such a reduction suffers
from an exponential blow up in the state size (commonly known as the
\textit{curse of history} \cite{pineau2003point}).  When inferring
tasks from demonstrations, where different hypotheses may have
different historical dependencies, na\"{i}vely encoding the entire
history quickly becomes intractable.

A second limitation relates to the \textit{compositionality} of task
representations. As suggested, Ex~\ref{ex:intro} naturally
decomposes into two sub-tasks. Ideally, we would want an algorithm
that could learn each sub-task and combine them into the complete
task, rather than only be able to learn single monolithic tasks.
However, for many classes of quantitative rewards, "combining" rewards
remains an ad-hoc procedure. The situation is further exacerbated by
humans being notoriously bad at anticipating or identifying when
quantitative rewards will lead to unintended consequences
\cite{ho_teaching_2015}, which poses a serious problem for AI
safety~\cite{amodei2016concrete} and has led to investigations into
reward repair~\cite{ghosh2018repair}. For instance, we could take a
linear combination of rewards for each of the subtasks in
Ex~\ref{ex:intro}, but depending on the relative scales of the
rewards, and temporal discount rate, wildly different behaviors would
result.

\begin{wrapfigure}{r}{4cm}
  \centering
  \begin{subfigure}{1.0\linewidth}
    \centering
    \def\svgwidth{3.2cm}
    \input{imgs/with-recharge.pdf_tex}
    \caption{\label{fig:yr}}
  \end{subfigure}
  \begin{subfigure}{1.0\linewidth}
    \centering
    \def\svgwidth{3.2cm}
    \input{imgs/missing-recharge.pdf_tex}
    \caption{\label{fig:bug}}
  \end{subfigure}
  \caption{Illustration of a bug in the learnt quantitative Markovian
    reward resulting from slight changes in the
    environment.\label{fig:brittle}}
\end{wrapfigure}
In fact, the third limitation - brittleness due to simple changes in
the environment - illustrates that often, the correctness of the agent
can change due to a simple change in the environment.  Namely, imagine
for a moment we remove the water and drying tiles from
Fig~\ref{fig:gridworld} and attempt to learn a reward that encodes the
``recharge while avoid lava'' task in
Ex~\ref{ex:intro}. Fig~\ref{fig:yr} illustrates the reward resulting
from performing Maximum Entropy Inverse Reinforcement
Learning~\cite{ziebart2008maximum} with the demonstrations shown in
Fig~\ref{fig:gridworld} and the binary features: red (lava tile),
yellow (recharge tile), and ``is wet''.  As is easy to verify, a
reward optimizing agent, $\sum_{i=0}^\infty \gamma^i r_i(s)$, with a
discount factor of $\gamma=0.69$ would generate the trajectory shown
in Fig~\ref{fig:yr} which avoids lava and eventually recharges.

Unfortunately, using the \emph{same} reward and discount factor on a
nearly identical world can result in the agent entering the lava. For
example, Fig~\ref{fig:bug} illustrates the learned reward being
applied to a change in the gridworld where the top left charging tile
has been removed. An acceptable trajectory is indicated via a dashed
arrow. Observe that now the discounted sum of rewards is maximized on
the solid arrow's path, resulting in the agent entering the lava! While
it is possible to find new discount factors to avoid this behavior,
such a supervised process would go against the spirit of automatically
learning the task.

Finally, we briefly remark that while non-Markovian Boolean rewards
cannot encode all possible rewards, e.g., ``run as fast as possible'',
often times such objectives can be reframed as policies for a Boolean
task. For example, consider modeling a race. If at each time step
there is a non-zero probability of entering a losing state, the agent
will run forward as fast as possible even for the Boolean task ``win
the race''.

Thus, quantitative Markovian rewards are limited as 
a task representation when learning tasks containing
\textit{temporal specifications} or \textit{compositionality} from
demonstrations.  Moreover, the need to fine tune learned tasks with
such properties seemingly undercuts the original purpose of learning
task representations that are generalizable and invariant to irrelevant
aspects of a task \cite{littman_environment-independent_2017}.

% Being able to learn tasks with \textit{temporal specifications} and 
% \textit{compositionality} 
% - history - explosion
% - compositionality - need to reweight

\textbf{Related Work:}
Our work is intimately related to Maximum Entropy
Inverse Reinforcement Learning. In Inverse Reinforcement Learning
(IRL)~\cite{ng2000algorithms} the demonstrator, operating in a
stochastic environment, is assumed to attempt to (approximately)
optimize some unknown reward function over the trajectories. In
particular, one traditionally assumes a trajectory's reward is the sum
of state rewards of the trajectory. This formalism offers a
succinct mechanism to encode and generalize the goals of the
demonstrator to new and unseen environments.

In the IRL framework, the problem of learning from demonstrations can
then be cast as a Bayesian inference
problem~\cite{ramachandran2007bayesian} to predict the most probable
reward function. To make this inference procedure well-defined and
robust to demonstration/modeling noise, Maximum Entropy
IRL~\cite{ziebart2008maximum} appeals to the principle of maximum
entropy~\cite{jaynes1957information}. This results in a likelihood
over the demonstrations which is no more committed to any particular
behavior than what is required for matching the empirically observed
reward expectation. While this approach was initially limited to
learning a linear combination of  feature vectors, IRL has been
successfully adapted to arbitrary function approximators such as
Gaussian processes~\cite{NIPS2011_4420} and neural
networks~\cite{finn2016guided}. As stated in the introduction,
while powerful, traditional IRL provides no principled mechanism
for composing the resulting rewards.

% Introduce Non-Markovian
To address this deficit, composition using soft optimality has recently
received a fair amount of attention; however, the compositions are
limited to either strict disjunction (do X \emph{or}
Y)~\cite{todorov2007linearly}~\cite{todorov2008general} or conjunction
(do X \emph{and} Y)~\cite{haarnoja2018composable}. Further, because soft
optimality only bounds the deviation from simultaneously optimizing
both rewards, optimizing the composition does not preclude violating
safety constraints embedded in the rewards (e.g., do not enter the
lava).

The closest work to ours is recent work on inferring Linear Temporal
Logic (LTL) by finding the specification that minimizes the expected
number of violations by an optimal agent compared to the expected
number of violations by an agent applying actions uniformly at
random~\cite{kasenberg2017interpretable}. The computation of the
optimal agent's expected violations is done via dynamic programming on
the explicit product of the deterministic Rabin
automaton~\cite{farwer2002omega} of the specification and the state
dynamics. A fundamental drawback to this procedure is that due to the
curse of history, it incurs a heavy run-time cost, even on simple two
state and two action Markov Decision Processes. We also note that the
literature on learning logical specifications from examples (e.g.,
\cite{jha2017telex,vazquez2017logical,Li:EECS-2014-20}), 
does not handle noise in examples while our
approach does.
Finally, once a specification has been identified, one can leverage
the rich literature on planning using temporal logic to synthesize a
policy~\cite{kress2009temporal,saha2014automated,raman2015reactive,jha2016automated,jha2018safe}.

\textbf{Contributions:}
(i) We formulate the problem of \emph{learning specifications from
demonstrations} in terms of Maximum a Posteriori inference. (ii) To
make this inference well defined, we appeal to the principle of
maximum entropy culminating in the distribution given
\eqref{eq:model}. The main contribution of this model is that it only
depends on the probability the demonstrator will successfully perform
task and the probability that the task is satisfied by performing
actions uniformly at random.  Because these properties can be
estimated without explicitly unrolling the dynamics in time, this
model avoids many of the pitfalls characteristic to the curse of
history. (iii) We provide an algorithm that exploits the piece-wise
convex structure in our posterior model~\eqref{eq:model} to
efficiently perform Maximum a Posteriori inference for the most
probable specification.

\textbf{Outline:} In Sec~\ref{sec:setup}, we define specifications and
probabilistic automata (Markov Decision Processes without rewards).
In Sec~\ref{sec:inference}, we introduce the problem of
\emph{specification inference from demonstrations}, and inspired by
Maximum Entropy IRL~\cite{ziebart2008maximum}, develop a model of the
posterior probability of a specification given a sequence of
demonstrations.  In Sec~\ref{sec:alg}, we develop an algorithm
to perform inference under~\eqref{eq:model}.  Finally, in Sec~\ref{sec:casestudies}, we demonstrate
how due to their inherent composability, learning specifications can
avoid common bugs that often occur due to ad-hoc reward composition.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> sections/spec_inference.sync-conflict-20180829-222004-WNN7ZOX.tex <==
\section{Background}\label{sec:setup}
We seek to learn specifications from demonstrations provided by a
teacher who executes a sequence of actions that probabilistically
changes the system state. For simplicity, we assume that the set of
actions and states are finite and fully observed. The system is
naturally modeled as a probabilistic automaton\footnote{In the
literature, a Probabilistic Automata are often denoted constructed as a
Markov Decision Process, $M$, without its Markovian reward map $R$, denoted $M \setminus R$.}
formally defined below:
\begin{definition}[Probabilistic Automaton]
  A probabilistic automaton is a tuple $ M = (S, s_0, A, \delta) $,
  where $ S $ is the finite set of states, $s_0 \in S$ is the initial
  state, $ A $ is the finite set of actions, and
  $ \delta : S \times A \times S \to [0, 1]$ specifies the transition
  probability of going from $ s $ to $ s' $ given action $ a $,
  i.e. $\delta(s, a, s') = \Prob(s'~|~s,a) $ and
  $\displaystyle \sum_{s'\in S} \Prob(s'~|~s,a) = 1$ for all states
  $s$.
\end{definition}

\begin{definition}[Trace]
  A sequence of state/action pairs is called a trace (or trajectory).
  A trace of length $\tau \in \Nat$ is an element of
  $(S \times A)^{\tau}$.
\end{definition}
Next, we develop machinery to distinguish between desirable and
undesirable traces. For simplicity, we focus on finite trace
properties, referred to as specifications, that are decidable within
some fixed $\tau \in \Nat$ time steps.  For example,
we do not allow ``eventually event A will occur,'' but do allow
``event A will occur before step 20.''  A specification, $\varphi$,
can be identified via its indicator function.
\begin{definition}[Specification]
  Given a set of states $S$, a set of actions $A$, and a fixed trace
length $\tau \in \Nat$, a specification, $\varphi$, is a predicate
over traces: $\varphi: (S \times A)^\tau \to \setof{0, 1}$. We define
  $\true(\xi) \eqdef 1$,
  $ \neg \varphi(\xi) \eqdef 1 - \varphi(\xi)$, $\false \eqdef \neg \true$.
  Finally, for convience, we abuse notation and denote by $\xi \in \varphi$
  the statement $\xi \in \setof{\xi\mid \varphi(\xi) = 1}$.
\end{definition}
Specifications may be given in formal notation, as sets, logical
formulas, or automata/monitors.
\thiswillnotshow{For our experiments, we focus on monitors induced
by temporal logical formula (see Fig~\ref{fig:monitor}).
\begin{figure}[h]
  \begin{center}\includegraphics[height=1.2in]{imgs/automata_picture.pdf}
    \caption{ Each specification records the sensor output each time
      an action is applied to the dynamical system and updates whether
      the specification is currently satisfied.  The composite monitor
      checks if specification 2 has held since the last time the
      first specification held or if specification 3 has held. An
      identical structure was used in the experiments to encode the
      constraint that either yellow was never stepped on, or brown was
      stepped on since the last time blue was stepped
      on.\label{fig:monitor}}
  \end{center}
\end{figure}
}
Further, the relation with logic facilitates defining a large suite of
non-trivial composition rules. For example, consider two
specifications, $\varphi_1$, $\varphi_2$ that encode tasks $A$ and $B$
resp and the composition rule $[\varphi_1 \wedge \varphi_2]: \xi
\mapsto \min\big (\varphi_1(\xi), \varphi_2(\xi)\big )$ which
implements logical AND.  Because the agent only receives a reward if
$\varphi_1(\xi) = \varphi_2(\xi) = 1$, then a reward optimizing agent
performs reward maximizing must necessarily perform tasks $A$ and $B$
simultaneously. Similarly, maximizing $[\varphi_1 \vee \varphi_2] :
\xi \mapsto \max\big(\varphi_1(\xi), \varphi_2(\xi)\big)$ corresponds
to logical OR. Using negation, one can then encode conditional
requirements. For example, maximizing $[\varphi_1 \implies \varphi_2]
: \xi \mapsto \max\big(\neg\varphi_1(\xi), \varphi_2(\xi)\big) =
\max\big(1 - \varphi_1(\xi), \varphi_2(\xi)\big)$ corresponds to only
requiring the agent to perform task B if task A is done.

Complicated temporal connectives can also be defined using temporal
logics~\cite{pnueli1977temporal} or
automata~\cite{vardi1996automata}). For our purposes, it suffices to
informally consider extending propositional logic with three temporal
operators: (1) Let $\square a$ denote that the state property $a$
holds at all time steps. (2) Let $\lozenge a \eqdef \neg (\square)$
denote that the property $a$ eventually holds. (3) Let $a~W~b$ denote
that the property $a$ holds at every time step until $b$ holds, and
$b$ is not required to ever hold. Crucially, temporal operators can be
composed to make more complicated sentences, although for time bounded
specifications these often For example, $\square (a \implies (b~W~c))$
translates to ``its always the case a implies b until c''. Observe
that the property BBY from the introductory example takes this exact
form, namely $\square (\text{blue} \implies (\neg
\text{yellow}~W~\text{brown}))$.


\section{Specification Inference}\label{sec:inference}
\begin{figure*}[!t]
  \begin{empheq}[box=\fbox]{align}\label{eq:model}\tag{$\star$}
      \mathcal{L}(\varphi~|~M, \Demos, \overline{\varphi},\alpha, \beta) =
  \overbrace{\rho_\Demos}^{\mathclap{\text{Probability of
        accidentally generating the demos.}}}
  + |\Demos|\cdot\underbrace{\KL\Big
    (\Bernoulli(\overline{\varphi})~\|~\Bernoulli(\widehat{\varphi})\Big
    )}_{\mathclap{\text{Information gain w.r.t. random action
        distribution.}}}
  + \overbrace{\ln\Big(\BetaDist(\overline{\varphi};
    \alpha, \beta)\Big)}^{\mathclap{\text{Bias towards positive
        demos.}}}
\end{empheq}
\end{figure*}

\begin{definition}[Specification Inference from
  Demonstrations]\label{problem1}
  The specification inference from demonstrations problem is a tuple
  $(M, \Demos, \Phi)$ where $M=(S, s_0, A, \delta) $ is a probabilistic
  automaton, $\Demos$ is a sequence of length-$\tau$ demonstrations drawn
  from an unknown distribution induced by some unknown specification,
  and $ \Phi \subseteq 2^{(S\times A)^\tau} $ is a family of
  specifications.  A solution to $(M, \Demos, \Phi)$ is:
  \begin{equation}
    \label{eq:RiskAverseProblem} \varphi^* \in \argmax_{\varphi \in \Phi}\Prob
    (\varphi~|~M, \Demos)\\
  \end{equation}
  where $\Prob(\varphi~|~M, \Demos,\Phi)$ denotes the probability that
  the teacher used specification $\varphi$ to generate demonstrations
  given that the demonstrations $\Demos$ were observed.
\end{definition}
To make this inference well-defined, we make a series of assumptions
on the form of the posterior. The resulting posterior model is given
in \eqref{eq:model}.

\noindent
\textbf{Likelihood of a demonstration:}
We begin by leveraging the principle of maximum entropy to
disambiguate the likelihood distributions. Concretely,
define
\begin{equation}
  \label{eq:trace_weight}
  w\big(\vec{\xi}=(\vec{s}, \vec{a}), M\big) = \prod_{i=0}^{\tau-1}\Prob(s_{i+1}|s_i, a_i, M)
\end{equation}
to be the weight of each possible demonstration $\xi$ induced by
automata $M$.  Given a demonstrator who on average satisfies the
specification $\varphi$ with probability $\overline{\varphi}$, we
approximate the likelihood function by:
\begin{equation}\label{eq:max_ent_dist}
    \Prob\big(\vec{\xi}~|~M, \varphi, \overline{\varphi}\big) = 
    w(\xi, M)\cdot \frac{\exp(\lambda_\varphi
      \varphi(\xi))}{Z_\varphi}
\end{equation} where $\vec{s}$ and $\vec{a}$ are the states and
actions of $\xi$ respectively and $\lambda_\varphi$, $Z_\varphi$ are
normalization factors such that $\Expected_\xi[\varphi] =
\overline{\varphi}$ and $\displaystyle \sum_\xi \Prob(\xi~|~M,\varphi)
=1$. \footnote{For some degenerate values of $\overline{\varphi}$, the
  derived model is the limit of taking $\lambda_\varphi$ to positive or
  negative infinity. One can easily check post-facto that the result is
  still the maximum entropy distribution.} For a detailed derivation that~\eqref{eq:max_ent_dist} is the maximimal entropy
distribution, we point the reader
to~\cite{DBLP:journals/corr/abs-1805-00909}. Next observe
that,~\eqref{eq:max_ent_dist} admits a simple closed form:
\begin{empheq}[box=\fbox]{align}\label{eq:max_ent_dist2}
  \Prob(\vec{\xi}~|~M, \varphi)=\widehat{\vec{\xi}}\cdot
  \begin{cases}
    \overline{\varphi}/\widehat{\varphi} & \xi \in \varphi\\
    \overline{\neg \varphi}/\widehat{\neg \varphi} & \xi \notin
    \varphi
  \end{cases}
\end{empheq}
where, in general, we will use a bar over a variable,
$\overline{(\cdot)}$, to indicate average w.r.t. $X$ and a hat,
$\widehat{(\cdot)}$, to denote expected value under random
actions. E.g., $\widehat{\vec{\xi}}$ is the probability of generating
trace $\xi$ with uniformly random actions and by the law
of the excluded middle:
$\widehat{\neg \varphi} = 1 - \widehat{\varphi}$ and
$\overline{\neg \varphi} = 1 - \overline{\varphi}$.
\begin{proof}
  For brevity, let
  $W_\varphi \eqdef \sum_{\vec{\xi} \in \varphi}
  w(\vec{\xi}, M)$ and $c \eqdef e^{\lambda_\varphi}$. Via the constraints
  on~\eqref{eq:max_ent_dist},
  \begin{equation}
    \begin{split}
      &Z_\varphi\cdot \overline{\varphi} = \sum_{\vec{\xi} \in \varphi} c\cdot w(\xi, M)
    = c W_\varphi\\
    &Z_\varphi = c \sum_{\vec{\xi} \in
      \varphi} w(\vec{\xi}, M) + \sum_{\vec{\xi} \notin \varphi} w(\vec{\xi},M) = c W_\varphi + W_{\neg \varphi}
    \end{split}
  \end{equation}
  Combining gives
  $Z_\varphi = W_{\neg \varphi}/\overline{\neg \varphi}$. Next,
  observe that if $\vec{\xi} \not \in \varphi$, then
  $e^{\lambda_\varphi \varphi(\xi)} = 1$ and substituting in~\eqref{eq:max_ent_dist} yields,
  \begin{equation} \Prob(\vec{\xi}~|~\varphi, M, \vec{x} \notin
    \varphi) = w_\xi\frac{\overline{\neg \varphi}}{W_{\neg \varphi}}
  \end{equation}
  If $\vec{\xi} \in \varphi$ (implying $W_\varphi \neq 0$) then
  $e^{\lambda_\varphi} = Z_\varphi (\overline{\varphi} / W_\varphi)$ then,
  \begin{equation} \Prob(\vec{\xi}~|~\varphi, M, \vec{\xi} \in
    \varphi) = w_\xi\frac{\overline{\varphi}}{W_\varphi}
  \end{equation}
  Finally, observe that
  $\widehat{\varphi} = \frac{W_\varphi}{W_{\text{true}}}$ and
  $\widehat{\vec{\xi}} =
  \frac{w_\vec{\xi}}{W_{\text{true}}}$. Substituting and factoring
  yields~\eqref{eq:max_ent_dist2}.
\end{proof}
\begin{proof}[Proof Sketch (proof in appendix)]
  Because $\varphi(\xi)$ can only take two values, ~\eqref{eq:max_ent_dist}
  can be decomposed as the sum of its $\varphi(\xi) = 1$ and $\varphi(\xi) = 1 - (\neg \phi(\xi)) = 0$ components. $Z$
  and $\lambda$ are then found via simple algebraic
  manipulations. Finally, observe that $\displaystyle\widehat{\varphi} = \frac{\sum_{\varphi(\xi) = 1} w(\xi)}{\sum_{\xi} w(\xi)}$.
  Substituting yields~\eqref{eq:max_ent_dist2}.
\end{proof}
\noindent
\textbf{Likelihood of a demonstration sequence:}
If the teacher gives a finite sequence of $\tau$ length
demonstrations, $\Demos$, drawn i.i.d. from~\eqref{eq:max_ent_dist2},
then the log likelihood, $\mathcal{L}$, of $\Demos$ is:
\begin{equation}\label{eq:max_ent_dist3}
  \mathcal{L(\Demos~|~M, \varphi, \overline{\varphi})} \approx \rho_\Demos+ N_\varphi \ln\left(\frac{\overline{\varphi}}{
    \widehat{\varphi}}\right)
    + N_{\neg\varphi} \ln\left(\frac{\overline{\neg\varphi}}{
    \widehat{\neg \varphi}}\right)
\end{equation}
where by definition we take $(0\cdot \ln( \ldots ) = 0)$ and:\footnote{ We
  have suppressed a multinomial coefficient required if any two
  demonstrations are the same.  However, since this term will not
  change as $\varphi$ varies, one can simply absorb this coefficient
  into $\rho(\Demos)$.}
\begin{equation}
  \rho_\Demos \eqdef \displaystyle \log\bigg (\prod_{\vec{\xi} \in \Demos}
  \widehat{\vec{\xi}}\bigg)~~~~~~~~
  N_\varphi \eqdef \sum_{\vec{\xi}\in \Demos} \varphi(\xi) \approx |\Demos|\overline{\varphi}
\end{equation}
Next, observe that
$\displaystyle \left[\overline{\varphi}\ln\left(\frac{\overline{\varphi}}
    {\widehat{\varphi}}\right) + (1 - \overline{\varphi})\ln\left(\frac{1 -
      \overline{\varphi}}{ 1 - \widehat{ \varphi}}\right)\right]$ is the
information gain (KL divergence) between two Bernoulli distributions with means
$\overline{\varphi}$ and $\widehat{\varphi}$ resp. Letting $\mathcal{B}(\mu)$
denote a Bernoulli distribution with mean $\mu$ and
$\displaystyle \KL(P~\|~Q) \eqdef \sum_{i}P(i) \ln(P(i)/Q(i))$
denote the information gain when using distribution
$P$ compared to $Q$, if $X$ is representative, we can approximate~\eqref{eq:max_ent_dist3} as:
\begin{empheq}[box=\fbox]{align}\label{eq:max_ent_dist5}
  \begin{split}
    \mathcal{L}(\Demos~|~M, \varphi, \overline{\varphi})\approx
    \rho_\Demos + |\Demos|\KL\left
      (\Bernoulli(\overline{\varphi})~\|~\Bernoulli(\widehat{\varphi})\right
)
  \end{split}
\end{empheq}
Unfortunately,~\eqref{eq:max_ent_dist5} has the following
undesirable symmetry:
\begin{equation}
  \Prob(\Demos~|~M, \varphi) = \Prob(\Demos~|~M, \neg \varphi)
\end{equation}
Intuitively, this symmetry derives from the fact that a specification can be
uniquely demonstrated as the set of all positive examples or as the
negation of the set of all negative examples.

We address this by explicitly modeling the ``competency'' of
the agent via a prior on $\overline{\varphi}$ that favors positive
demonstrations ($\overline{\varphi}$ near 1). As $\overline{\varphi}$ lies
strictly within 0 and 1, we model the prior over
$\overline{\varphi}$ with a beta distribution with $\beta\approx 1$ and
$\alpha > 3$ which biases towards positive demonstrations.
\begin{equation}
  \begin{split}
    \Prob(\overline{\varphi} = \theta ~|~M, \varphi, \alpha, \beta)  &\eqdef \BetaDist(\theta; \alpha, \beta)\\
    &\propto \theta^{\alpha - 1}(1 - \theta)^{\beta - 1}    
  \end{split}
\end{equation}

Further assuming a uniform prior on $\varphi$, we arrive at the
posterior distribution given in~\eqref{eq:model}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> spec_inference.tex <==
\vspace{-10px}
\section{Background}\label{sec:setup}
We seek to learn specifications from demonstrations provided by a
teacher who executes a sequence of actions that probabilistically
changes the system state. For simplicity, we assume that the set of
actions and states are finite and fully observed. The system is
naturally modeled as a probabilistic automaton\footnote{Probabilistic Automata are often constructed as a
Markov Decision Process, $M$, without its Markovian reward map $R$, denoted $M \setminus R$.}
formally defined below:
\begin{mddef}[Probabilistic Automaton]
  A \textbf{probabilistic automaton} is a tuple $ M = (S, s_0, A, \delta) $,
  where $ S $ is the finite set of states, $s_0 \in S$ is the initial
  state, $ A $ is the finite set of actions, and
  $ \delta : S \times A \times S \to [0, 1]$ specifies the transition
  probability of going from $ s $ to $ s' $ given action $ a $,
  i.e. $\delta(s, a, s') = \Prob(s'~|~s,a) $ and
  $\displaystyle \sum_{s'\in S} \Prob(s'~|~s,a) = 1$ for all states
  $s$.
\end{mddef}

\begin{mddef}[Trace]
  A sequence of state/action pairs is called a \textbf{trace}
  (trajectory, demonstration).  A trace of length $\tau \in \Nat$ is
  an element of $(S \times A)^{\tau}$.
\end{mddef}
Next, we develop machinery to distinguish between desirable and
undesirable traces. For simplicity, we focus on finite trace
properties, referred to as specifications, that are decidable within
some fixed $\tau \in \Nat$ time steps, e.g., ``event A occurred in the
last 20 steps''.
\begin{mddef}[Specification]
  Given a set of states $S$, a set of actions $A$, and a fixed trace
  length $\tau \in \Nat$, a \textbf{specification} is a subset of
  traces $\varphi \subseteq (S \times A)^\tau$. We define
  $\true \eqdef (S \times A)^\tau$,
  $\neg \varphi \eqdef \true \setminus \varphi$, and
  $\false \eqdef \neg \true$. A collection
  of specifications, $\Phi$, is called a \textbf{concept class}.
  Finally, we abuse notation and use
  $\varphi$ to also denote its indicator function (interpreted as a non-Markovian Boolean reward),
  \begin{equation}
    \varphi(\xi) \eqdef 
    \begin{cases}
      1 & \text{if } \xi \in \varphi\\
      0 & \text{otherwise}
    \end{cases}
    .
  \end{equation}
\end{mddef}
Specifications may be given in formal notation, as sets or
automata. Further, each representation facilitates defining a
plethora of composition rules. For example, consider two specifications,
$\varphi_A$, $\varphi_B$ that encode tasks $A$ and $B$ respectively
and the composition rule $\varphi_A \cap \varphi_B: \xi \mapsto
\min\big (\varphi_A(\xi), \varphi_B(\xi)\big )$. Because the agent
only receives a non-zero reward if $\varphi_A(\xi) = \varphi_B(\xi) = 1$, a
reward maximizing agent must necessarily perform tasks $A$ and $B$
simultaneously. Thus, $\varphi_A \cap \varphi_B$ corresponds to
conjunction (logical \emph{and}). Similarly, maximizing $\varphi_A \cup
\varphi_B : \xi \mapsto \max\big(\varphi_A(\xi), \varphi_B(\xi)\big)$
corresponds to disjunction (logical \emph{or}). One can also encode
conditional requirements using subset inclusion, e.g.,
maximizing $\varphi_A \subseteq \varphi_B : \xi \mapsto
\max\big(1 - \varphi_A(\xi), \varphi_B(\xi)\big)$ corresponds to
task A triggering task B.

Complicated temporal connectives can also be defined using temporal
logics~\cite{pnueli1977temporal} or
automata~\cite{vardi1996automata}. For our purposes, it suffices to
informally extend propositional logic with three temporal
operators: (1) Let $H a$, read ``historically $a$'', denote that property $a$ held at all previous time steps. (2) Let $P a \eqdef \neg (H
\neg a)$, read ``once $a$'', denote that the property $a$ 
at least once held in the past. (3) Let $a~S~b$, read ``$a$ since $b$'', denote that the property
$a$ that has held every time step after $b$ last held. The true power
of temporal operators is realized when they are composed to make more
complicated sentences. For example, $H (a \implies (b~S~c))$
translates to ``it was always the case that if $a$ was true, then
$b$ has held since the last time $c$ held.''. Observe that the property BBY from the introductory example
takes this form, $H ((\text{yellow} \wedge P~\text{blue}) \implies
(\neg \text{blue}~S~\text{brown}))$, i.e., ``Historically, if the agent had once visited blue and is currently visiting yellow, then the agent has not visited blue since it last visited brown''.

\section{Specification Inference from Demonstrations}\label{sec:inference}
\vspace{-5px}
In the spirit of Inverse Reinforcement Learning, we now seek to
find the specification that best explains the behavior of the
agent. We refer to this as \emph{Specification Inference from Demonstrations}.
\begin{mddef}[Specification Inference from
  Demonstrations]\label{problem1}
  The \textbf{specification inference from demonstrations} problem is a tuple
  $(M, \Demos, \Phi)$ where $M=(S, s_0, A, \delta) $ is a
  probabilistic automaton, $\Demos$ is a (multi-)set of $\tau$-length
  traces drawn from an unknown distribution induced by a teacher
  attempting to demonstrate some unknown specification within $M$, and $ \Phi $ a
  concept class of specifications. 
  
  A solution to
  $(M, \Demos, \Phi)$ is:
  \begin{equation}
    \label{eq:RiskAverseProblem} \varphi^* \in \argmax_{\varphi \in \Phi}\Prob
    (\varphi~|~M, \Demos)\\
  \end{equation}
  where $\Prob(\varphi~|~M, \Demos)$ denotes the probability that
  the teacher demonstrated $\varphi$
  given the observed traces, $\Demos$, and the dynamics, $M$.
\end{mddef}
To make this inference well-defined, we make a series of assumptions
culminating in \eqref{eq:model}.

\textbf{Likelihood of a demonstration:}
We begin by leveraging the principle of maximum entropy to
disambiguate the likelihood distributions. Concretely,
define:
\begin{equation}
  \label{eq:trace_weight}
  w\big(\vec{\xi}=(\vec{s}, \vec{a}), M\big) = \prod_{i=0}^{\tau-1}\Prob(s_{i+1}|s_i, a_i, M)
\end{equation} where $\vec{s}$ and $\vec{a}$ are the 
projected sequences of states and
actions of $\xi$ respectively,
to be the weight of each possible demonstration $\xi$ induced by
dynamics $M$.  Given a demonstrator who on average satisfies the
specification $\varphi$ with probability $\overline{\varphi}$, we
approximate the likelihood function by:
\begin{equation}\label{eq:max_ent_dist}
    \Prob\big(\vec{\xi}~|~M, \varphi, \overline{\varphi}\big) = 
    w(\xi, M)\cdot \frac{\exp(\lambda_\varphi
      \varphi(\xi))}{Z_\varphi}
\end{equation} where $\lambda_\varphi$, $Z_\varphi$ are
normalization factors such that $\Expected_\xi[\varphi] =
\overline{\varphi}$ and $\sum_\xi \Prob(\xi~|~M,\varphi)
=1$. For a detailed derivation that~\eqref{eq:max_ent_dist} is the maximal entropy
distribution, we point the reader
to~\cite{DBLP:journals/corr/abs-1805-00909}. Next observe
that due to the Boolean nature of $\varphi$,~\eqref{eq:max_ent_dist} admits a simple closed form:
\begin{empheq}[box=\fbox]{align}\label{eq:max_ent_dist2}
  \Prob(\vec{\xi}~|~M, \varphi, \overline{\varphi})=\widetilde{\setof{\vec{\xi}}}\cdot
  \begin{cases}
    \overline{\varphi}/\widetilde{\varphi} & \xi \in \varphi\\
    (1 - \overline{\varphi})/\widetilde{\neg \varphi} & \xi \notin
    \varphi
  \end{cases}
\end{empheq}
where in general we use $\widetilde{(\cdot)}$ to denote the probability of
satisfying a specification using uniformly random actions. Thus, we denote by $\widetilde{\setof{\vec{\xi}}}$ the probability of randomly generating demonstration $\xi$
within $M$. Further, note that by the law of the excluded middle, for any specification:
$\widetilde{\neg \varphi} = 1 - \widetilde{\varphi}$.

\begin{proof}[Proof Sketch]
  For brevity, let
  $W_\varphi \eqdef \sum_{\vec{\xi} \in \varphi}
  w(\vec{\xi}, M)$ and $c \eqdef e^{\lambda_\varphi}$. Via the constraints
  on~\eqref{eq:max_ent_dist},
  \begin{equation}
    \begin{split}
      &Z_\varphi\cdot \overline{\varphi} = 1\cdot\sum_{\vec{\xi} \in \varphi} c^1\cdot w(\xi, M) + 0\cdot\sum_{\vec{\xi} \notin \varphi} c^0\cdot w(\xi, M)
    = c W_\varphi\\
    &Z_\varphi = c^1 \sum_{\vec{\xi} \in
      \varphi} w(\vec{\xi}, M) + c^0\sum_{\vec{\xi} \notin \varphi} w(\vec{\xi},M) = c W_\varphi + W_{\neg \varphi}
    \end{split}
  \end{equation}
  Combining gives
  $Z_\varphi = W_{\neg \varphi}/(1 - \overline{\varphi})$. Next,
  observe that if $\vec{\xi} \not \in \varphi$, then
  $e^{\lambda_\varphi \varphi(\xi)} = 1$ and substituting in~\eqref{eq:max_ent_dist} yields,
  $\displaystyle\Prob(\vec{\xi}~|~\varphi, M, \vec{\xi} \notin
    \varphi) = w_\xi(1 - \overline{\varphi})/ W_{\neg \varphi}$.
  If $\vec{\xi} \in \varphi$ (implying $W_\varphi \neq 0$) then
  $e^{\lambda_\varphi} = Z_\varphi \overline{\varphi} / W_\varphi$ and
  $\displaystyle \Prob(\vec{\xi}~|~\varphi, M, \vec{\xi} \in
  \varphi) = w_\xi\overline{\varphi}/ W_\varphi$.
  Finally, observe that
  $\widetilde{\varphi} = W_\varphi/ W_{\text{true}}$ and
  $\widetilde{\setof{\vec{\xi}}} =
  w_\vec{\xi}/ W_{\text{true}}$. Substituting and factoring
  yields~\eqref{eq:max_ent_dist2}.
\end{proof}  

\textbf{Likelihood of a set of demonstrations:}
If the teacher gives a finite sequence of $\tau$ length
demonstrations, $\Demos$, drawn i.i.d. from~\eqref{eq:max_ent_dist2},
then the log likelihood, $\mathcal{L}$, of $\Demos$ under~\eqref{eq:max_ent_dist2} is:\footnote{ We
  have suppressed a multinomial coefficient required if any two
  demonstrations are the same.  However, this term will not
  change as $\varphi$ varies, and thus cancels when comparing across specifications.}
\begin{equation}\label{eq:max_ent_dist3}
  \mathcal{L}(\Demos~|~M, \varphi, \overline{\varphi}) = \displaystyle \log\bigg (\prod_{\vec{\xi} \in \Demos}
  \widetilde{\setof{\vec{\xi}}}\bigg) + N_\varphi \ln\left(\frac{\overline{\varphi}}{
    \widetilde{\varphi}}\right)
    + N_{\neg\varphi} \ln\left(\frac{\overline{\neg\varphi}}{
    \widetilde{\neg \varphi}}\right)
\end{equation}
where by definition we take $(0\cdot \ln( \ldots ) = 0)$ and $\displaystyle N_\varphi \eqdef \sum_{\vec{\xi}\in \Demos} \varphi(\xi)$.

Next, observe that
$\displaystyle \left[\overline{\varphi}\ln\left(\frac{\overline{\varphi}}
    {\widetilde{\varphi}}\right) + (1 - \overline{\varphi})\ln\left(\frac{1 -
      \overline{\varphi}}{ 1 - \widetilde{ \varphi}}\right)\right]$ is the
information gain (KL divergence) between two Bernoulli distributions with means
$\overline{\varphi}$ and $\widetilde{\varphi}$ resp. Syntactically, let $\mathcal{B}(\mu)$
denote a Bernoulli distribution with mean $\mu$ and
$\displaystyle \KL(P~\|~Q) \eqdef \sum_{i}P(i) \ln(P(i)/Q(i))$
denote the information gain when using distribution
$P$ compared to $Q$. If $X$ is ``representative'' such that $N_\varphi \approx \overline{\varphi}\cdot|\Demos|$, we can (up to a $\varphi$ independent normalization) approximate~\eqref{eq:max_ent_dist3}:
\begin{equation}\label{eq:max_ent_dist5}
  \Prob(\Demos~|~M, \varphi, \overline{\varphi})\appropto
  \exp{\Big(|\Demos|\cdot \KL\Big
      (\Bernoulli(\overline{\varphi})~\|~\Bernoulli(\widetilde{\varphi})\Big
)\Big)}  
\end{equation}
Where $\appropto$ denotes approximately proportional to.
Unfortunately, the approximation $|\Demos|\cdot \overline{\varphi}
\approx N_\phi$ implies that, $\overline{\neg \varphi} = 1 -
\overline{\varphi}$ which introduces the undesirable symmetry,
$\Prob(\Demos~|~M, \varphi, \overline{\varphi}) = \Prob(\Demos~|~M,
\neg \varphi, \overline{\neg \varphi})$,
into~\eqref{eq:max_ent_dist5}. To break this
symmetry, we assert that the demonstrator must
be at least as good as random. Operationally, we assert that
$\Prob(\varphi~|~\overline{\varphi} < \widetilde{\varphi}) = 0$ and is
otherwise uniform. Finally, we arrive at the posterior distribution given
in~\eqref{eq:model}, where $\mathbf{1}[\cdot]$ denotes an indicator function.
\begin{empheq}[box=\fbox]{align}\label{eq:model}
  ~~\Prob(\varphi~|~M, \Demos, \overline{\varphi}) \appropto \overbrace{\mathbf{1}[\overline{\varphi}\geq \widetilde{\varphi}]}^{\mathclap{\text{Demonstrator is better than random.}}}\cdot\exp\big(
      |\Demos|\cdot\overbrace{\KL\left
    (\Bernoulli(\overline{\varphi})~\|~\Bernoulli(\widetilde{\varphi})\right
    )}^{\mathclap{\text{Information gain over random actions.}}}
  \big)~~
\end{empheq}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

